Are Triggering Rates of Labquakes Universal? Inferring Triggering Rates From Incomplete Information

The acoustic emission activity associated with recent rock fracture experiments under different conditions has indicated that some features of event-event triggering are independent of the details of the experiment and the materials used and are often even indistinguishable from tectonic earthquakes. While the event-event triggering rates or aftershock rates behave pretty much identical for all rock fracture experiments at short times, this is not the case for later times. Here, we discuss how these differences can be a consequence of the aftershock identification method used and show that the true aftershock rates might have two distinct regimes. Specifically, tests on a modified Epidemic Type Aftershock Sequence model show that the model rates cannot be correctly inferred at late times based on temporal information only if the activity rates or the branching ratio are high. We also discuss both the effect of the two distinct regimes in the aftershock rates and the effect of the background rate on the inter-event time distribution. Our findings should be applicable for inferring event-event triggering rates for many other types of triggering and branching processes as well.

==> figs/scaled_M1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5241.60,4665.60)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(488,1284){\makebox(0,0)[r]{\strut{}$10^{-10}$}}%
      \put(488,2296){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \put(488,3307){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(488,4319){\makebox(0,0)[r]{\strut{}$10^{5}$}}%
      \put(1302,255){\makebox(0,0){\strut{}${-10}$}}%
      \put(2236,255){\makebox(0,0){\strut{}${-5}$}}%
      \put(3170,255){\makebox(0,0){\strut{}${0}$}}%
      \put(4105,255){\makebox(0,0){\strut{}${5}$}}%
      \put(5039,255){\makebox(0,0){\strut{}${10}$}}%
      \put(-282,2397){\rotatebox{-270}{\makebox(0,0){\strut{}$\frac{{x}_c}{k} 10^{-{\alpha} m_0}  \widehat{\phi}({\tau}|m_0)$}}}%
      \put(2796,57){\makebox(0,0){\strut{}$\log_{10}({\tau}/{x_c})-0.5m_0$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(963,1392){\makebox(0,0)[l]{\strut{}$\widetilde{\phi}(\theta_1,{\theta}_2)$}}%
      \csname LTb\endcsname%
      \put(963,1106){\makebox(0,0)[l]{\strut{}$n_b=0.2$}}%
      \csname LTb\endcsname%
      \put(963,820){\makebox(0,0)[l]{\strut{}$n_b=0.95$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{scaled_M1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/scaled_MAS.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6768.00,7056.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,4278){\makebox(0,0)[r]{\strut{}$10^{-10}$}}%
      \put(726,5036){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \put(726,5793){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(726,6551){\makebox(0,0)[r]{\strut{}$10^{5}$}}%
      \put(1272,3452){\makebox(0,0){\strut{}}}%
      \put(1872,3452){\makebox(0,0){\strut{}}}%
      \put(2471,3452){\makebox(0,0){\strut{}}}%
      \put(3071,3452){\makebox(0,0){\strut{}}}%
      \put(3671,3452){\makebox(0,0){\strut{}}}%
      \put(-44,5111){\rotatebox{-270}{\makebox(0,0){\strut{}$\frac{x_c}{k} 10^{-{\alpha} m_0}  \widehat{{\Phi}_{c}}({\tau}|m_0)$}}}%
      \put(2231,6771){\makebox(0,0){\strut{}$n_b=0.20$}}%
      \put(3311,6248){\makebox(0,0)[l]{\strut{}(a)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1181,3967){\makebox(0,0)[l]{\strut{}$\phi (\theta_1,\theta_2)$}}%
      \csname LTb\endcsname%
      \put(1181,4253){\makebox(0,0)[l]{\strut{}$\Phi_c (\theta_1, n_b)$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3678,4278){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,5036){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,5793){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,6551){\makebox(0,0)[r]{\strut{}}}%
      \put(4224,3452){\makebox(0,0){\strut{}}}%
      \put(4824,3452){\makebox(0,0){\strut{}}}%
      \put(5423,3452){\makebox(0,0){\strut{}}}%
      \put(6023,3452){\makebox(0,0){\strut{}}}%
      \put(6623,3452){\makebox(0,0){\strut{}}}%
      \put(3788,5111){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \put(5183,6771){\makebox(0,0){\strut{}$n_b=0.95$}}%
      \put(6263,6248){\makebox(0,0)[l]{\strut{}(b)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,1325){\makebox(0,0)[r]{\strut{}$10^{-10}$}}%
      \put(726,2083){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \put(726,2841){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(726,3599){\makebox(0,0)[r]{\strut{}$10^{5}$}}%
      \put(1272,587){\makebox(0,0){-10}}%
      \put(1872,587){\makebox(0,0){-5}}%
      \put(2471,587){\makebox(0,0){0}}%
      \put(3071,587){\makebox(0,0){5}}%
      \put(3671,587){\makebox(0,0){10}}%
      \put(-44,2159){\rotatebox{-270}{\makebox(0,0){\strut{}$\frac{x_c}{k} 10^{-{\alpha} m_0}   \mathrm{MAS}({\tau}|m_0)$}}}%
      \put(2231,301){\makebox(0,0){\strut{}$\log_{10}({\tau}/{x_c})-0.5m_0$}}%
      \put(3311,3296){\makebox(0,0)[l]{\strut{}(c)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1181,1014){\makebox(0,0)[l]{\strut{}$\widehat{\Phi_c} (x_c) - \langle{\mu}\rangle$}}%
      \csname LTb\endcsname%
      \put(1181,1300){\makebox(0,0)[l]{\strut{}$x_c$=10$^{-8}$}}%
      \csname LTb\endcsname%
      \put(1181,1586){\makebox(0,0)[l]{\strut{}$x_c$=0.0167}}%
      \csname LTb\endcsname%
      \put(1181,1872){\makebox(0,0)[l]{\strut{}$x_c$=1}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3678,1325){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,2083){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,2841){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,3599){\makebox(0,0)[r]{\strut{}}}%
      \put(4224,587){\makebox(0,0){-10}}%
      \put(4824,587){\makebox(0,0){-5}}%
      \put(5423,587){\makebox(0,0){0}}%
      \put(6023,587){\makebox(0,0){5}}%
      \put(6623,587){\makebox(0,0){10}}%
      \put(3788,2159){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \put(5183,301){\makebox(0,0){\strut{}$\log_{10}({\tau}/{x_c})-0.5m_0$}}%
      \put(6263,3296){\makebox(0,0)[l]{\strut{}(d)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{scaled_MAS}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/scaled_MAS2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6768.00,4104.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,719){\makebox(0,0)[r]{\strut{}$10^{-6}$}}%
      \put(726,1439){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \put(726,2159){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \put(726,2879){\makebox(0,0)[r]{\strut{}$10^{-3}$}}%
      \put(726,3599){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(1152,587){\makebox(0,0){-3}}%
      \put(2232,587){\makebox(0,0){0}}%
      \put(3311,587){\makebox(0,0){3}}%
      \put(-110,2159){\rotatebox{-270}{\makebox(0,0){\strut{}$\frac{{x}_c}{k} 10^{-{\alpha} m_0}   {\Phi}({\tau}|m_0)$}}}%
      \put(2231,301){\makebox(0,0){\strut{}$\log_{10}({\tau}/{x_c})-0.5m_0$}}%
      \put(2231,3819){\makebox(0,0){\strut{}$\sigma=1.00$}}%
      \put(3123,3223){\makebox(0,0)[l]{\strut{}(a)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1277,925){\makebox(0,0)[l]{\strut{}${\tau}^{-0.28(2)}$}}%
      \csname LTb\endcsname%
      \put(1277,1211){\makebox(0,0)[l]{\strut{}$\widehat{\Phi_{c}}$}}%
      \csname LTb\endcsname%
      \put(1277,1497){\makebox(0,0)[l]{\strut{}${\mathrm{MAS}}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3678,719){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,1439){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,2159){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,2879){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,3599){\makebox(0,0)[r]{\strut{}}}%
      \put(4104,587){\makebox(0,0){-3}}%
      \put(5184,587){\makebox(0,0){0}}%
      \put(6263,587){\makebox(0,0){3}}%
      \put(3590,2159){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \put(5183,301){\makebox(0,0){\strut{}$\log_{10}({\tau}/{x_c})-0.5m_0$}}%
      \put(5183,3819){\makebox(0,0){\strut{}$\sigma=3.00$}}%
      \put(6075,3223){\makebox(0,0)[l]{\strut{}(b)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{scaled_MAS2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/scaled_WT.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6696.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,719){\makebox(0,0)[r]{\strut{}$10^{-15}$}}%
      \put(726,1439){\makebox(0,0)[r]{\strut{}$10^{-10}$}}%
      \put(726,2159){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \put(726,2879){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(726,3599){\makebox(0,0)[r]{\strut{}$10^{5}$}}%
      \put(984,565){\makebox(0,0){\strut{}$10^{-5}$}}%
      \put(1944,565){\makebox(0,0){\strut{}$10^{0}$}}%
      \put(2903,565){\makebox(0,0){\strut{}$10^{5}$}}%
      \put(-57,2159){\rotatebox{-270}{\makebox(0,0){\strut{}$\langle{\delta}\rangle \mathrm{DWT}({\delta})$}}}%
      \put(2231,345){\makebox(0,0){\strut{}${\delta}/\langle{\delta}\rangle$}}%
      \put(2231,3819){\makebox(0,0){\strut{}${\sigma}=1.00$}}%
      \put(3287,3311){\makebox(0,0)[l]{\strut{}(a)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1317,925){\makebox(0,0)[l]{\strut{}$x_c=10^{-8}$}}%
      \csname LTb\endcsname%
      \put(1317,1211){\makebox(0,0)[l]{\strut{}$x_c=0.0167$}}%
      \csname LTb\endcsname%
      \put(1317,1497){\makebox(0,0)[l]{\strut{}$x_c=1$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3678,719){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,1439){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,2159){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,2879){\makebox(0,0)[r]{\strut{}}}%
      \put(3678,3599){\makebox(0,0)[r]{\strut{}}}%
      \put(3936,565){\makebox(0,0){\strut{}$10^{-5}$}}%
      \put(4896,565){\makebox(0,0){\strut{}$10^{0}$}}%
      \put(5855,565){\makebox(0,0){\strut{}$10^{5}$}}%
      \put(3774,2159){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \put(5183,345){\makebox(0,0){\strut{}${\delta}/\langle{\delta}\rangle$}}%
      \put(5183,3819){\makebox(0,0){\strut{}$\sigma=3.00$}}%
      \put(6239,3311){\makebox(0,0)[l]{\strut{}(b)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4269,925){\makebox(0,0)[l]{\strut{}$\langle{\delta}\rangle {\phi}(\frac{{\delta}}{\langle{\delta}\rangle})/k$}}%
      \csname LTb\endcsname%
      \put(4269,1211){\makebox(0,0)[l]{\strut{}${\delta}^{-2.5}$}}%
      \csname LTb\endcsname%
      \put(4269,1497){\makebox(0,0)[l]{\strut{}${\delta}^{-1.41}$}}%
      \csname LTb\endcsname%
      \put(4269,1783){\makebox(0,0)[l]{\strut{}${\delta}^{-0.66}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{scaled_WT}}%
    \gplfronttext
  \end{picture}%
\endgroup

